MetaLint: Easy-to-Hard Generalization for Code Linting

Large language models excel at code generation but struggle with code linting, particularly in generalizing to unseen or evolving best practices beyond those observed during training. We introduce MetaLint, a meta-learning framework that formulates code linting as an instruction-following task, where a model evaluates whether code adheres to a natural language specification of best practices. In contrast to prior work that trains models to detect violations from a fixed set of best practices, MetaLint evaluates code against a provided natural language specification, enabling test-time control over which practices to enforce and generalization to unseen or evolving rules without retraining. We demonstrate that models trained solely on synthetic data generated from automatic linters still generalize to harder, context-dependent best practices for which such linters are not available. To evaluate generalization beyond such easy signals, we introduce a human-curated benchmark of hard best practices inspired by Python Enhancement Proposals (PEPs). On this benchmark, MetaLint substantially improves performance without explicit fine-tuning on target best practices and exhibits strong, easy-to-hard generalization. Qwen3-4B achieves a 2.7x detection F-score gain (25.9% -> 70.4%), the highest recall, and a 26.7% localization F-score, matching larger models such as o3-mini. These gains generalize across programming languages, model families, scales, reasoning settings, and linter sources. We release the code and benchmark to support reproducibility and future work.

==> sections/000_abstract.tex <==
Large language models excel at code generation but struggle with code linting, particularly in generalizing to unseen or evolving best practices beyond those observed during training.
% \yiqing{you probably want to explain what is "static training data" in another way. Do you mean code linting is challenging, and generalizing to unseen lint rules is even more challenging? Can we say that most existing works only train on a fixed set of lint rules?}
% We introduce \textsc{MetaLint}, a training framework that formulates code linting as detecting best-practice violations from high-level specifications over semantic code fragments (code idioms).
We introduce \textsc{MetaLint}, a framework that formulates code linting as detecting violations of high-level best-practice specifications.
% \yiqing{detecting semantic code fragments that violate high-level specifications?}
To generalize beyond a fixed set of lint rules, \textsc{MetaLint} reorganizes supervision around dynamically specified best practices using synthetic linter-derived labels, integrated with instruction-following and preference optimization.
This encourages extrapolation to more complex, unseen best practices at test time, enabling easy-to-hard generalization without retraining.
To evaluate \textsc{MetaLint}, we introduce a benchmark of hard-to-detect best practices inspired by Python Enhancement Proposals (PEPs).
On this benchmark, \textsc{MetaLint} improves generalization to best practices without explicit fine-tuning on them.
Qwen3-4B achieves a 2.7× detection F-score gain (25.9\% → 70.4\%), the highest recall, and a 26.7\% localization F-score, matching larger models such as o3-mini.
These gains generalize across programming languages, model families, scales, reasoning settings, and linter sources.
We release the code and benchmark to support reproducibility and future work.

==> sections/000_abstract_old.tex <==
    Large Language Models, though successful in code generation, struggle with code quality analysis because they are limited by static training data and can't easily adapt to evolving best practices.
    % \law{The opening sentence is sounding too broad, maybe we can do better framing? for example the word narrow isn't conveying the proper meaning.}  
    We introduce \textsc{MetaLint}, a new instruction-following framework that formulates code quality analysis as the task of detecting and fixing problematic semantic code fragments or \textit{code idioms} based on high-level specifications. 
    Unlike conventional approaches that train models on static, rule-based data, \textsc{MetaLint} employs instruction tuning on synthetic linter-generated data to support easy-to-hard generalization, enabling models to adapt to novel or complex code patterns without retraining. To evaluate this, we construct a benchmark of challenging idioms inspired by real-world coding standards such as Python Enhancement Proposals (PEPs) and assess whether \textsc{MetaLint}-trained models reason adaptively or simply memorize. 
    % Our results show that \textsc{MetaLint} improves generalization to unseen PEP idioms, achieving 70.37\% F-score on idiom detection and 26.73\% on localization, competitive for its 4B parameter size and comparable to much larger state-of-the-art code and reasoning models like o3-mini, highlighting its potential for future-proof code quality analysis.
    Our results show that \textsc{MetaLint} improves generalization to unseen PEP idioms, achieving a 70.37\% F-score on idiom detection with the highest recall (70.43\%) among all evaluated models. 
    It also achieves 26.73\% on localization, competitive for its 4B parameter size and comparable to larger state-of-the-art models like o3-mini, highlighting its potential for future-proof code quality analysis.

==> sections/001_intro_v1.tex <==
\section{Introduction}
\textit{Code linting}, or static analysis to ensure code complies with best practices, offers a unique setting to study generalization in large language models (LLMs), as best practices constantly evolve and are poorly captured by static training data.
\yiqing{It's a little weird to mention "static training data" before introducing existing works? The flow can be: (1) introduce what's code linting, (2) existing works show benefits by training with fixed lint rules, (3) however, linting best practices evolve all the time (probably need some evidence). (4) training on static data does not reliably generalize to unseen best practices.}
Researchers have explored LLMs’ potential for best-practice-oriented linting \citep{vijayvergiya2024ai, fang2025lintllmopensourceveriloglinting, holden2024code, khare2023understanding, zhang2024refactoring}, and while they show benefits over rule-based linters, LLMs often end up memorizing specific best practices seen during training.
As a result, these systems often perform poorly on rare best practices, unseen code distributions \citep{holden2024code}, or over-flag outdated best practices, leading to negative user experiences and wasted time \citep{vijayvergiya2024ai}.
This difficulty stems not only from limited or outdated training data, but also from the way models are supervised: they are trained on a fixed set of best-practice labels, which encourages memorization of individual rules rather than learning generalizable abstractions.
More broadly, generalization to more complex or novel violations depends less on model scale or optimization, and more on how the learning problem is structured \citep{chang2025model}.

\yiqing{The structure of the introduction is a bit confusing to me. You talk about the reframing, your method, some challengings, cite some existing works, and go back to your method. Can we reorganize the pieces a little bit?}
\yiqing{Like, we first talk about reframing code linting to a meta-learning problem. Then we mention that training generalizable methods is challenging because some practices are easy and some are hard. In the next paragraph, we briefly motivate our idea from Yingshan's work (we can probably be more concise about this). After that, we use one paragraph to talk about the MetaLint framework (based on the motivation, we present MetaLint, ...). We can probably remove the "key contributions" paragraph and instead use one paragraph to show experiment results.}

Motivated by this view, rather than linting according to a fixed set of best practices, \textbf{we reframe code linting as meta-learning over \textit{code idioms}}: recurring patterns that capture semantic intent beyond surface syntax.
Here, we define best practices as semantic patterns over idioms, and violations occur when problematic idioms appear in contexts with safer or more appropriate alternatives (see Appendix~\ref{sec:appendix:term_definitions}).
We operationalize this by using linters to generate synthetic supervision for idioms, and train LLMs to detect and locate violations from high-level natural language specifications and examples (see Figure~\ref{fig:meta_lint_training_framework_part1}).
Code idioms provide a natural intermediate abstraction, bridging syntactic cues and full program semantics, enabling models to detect more complex, context-dependent best practices.
For example, in Python, generating passwords or tokens with \texttt{random.choice} is common but insecure in security-sensitive contexts.
PEP 506 \citep{pep506} recommends \texttt{secrets.choice} instead.
Detecting such violations requires conditional reasoning: not every \texttt{random.choice} is unsafe, but its use in security-critical code constitutes a violation.
Our approach trains models to recognize both the idiom (\texttt{random.choice}) and its context, enabling them to flag violations beyond simple syntactic patterns.

This illustrates a broader learning challenge.
Some best practices are relatively \textbf{easy to detect}, as they rely on surface-level cues.
For example, linters like Ruff include rules (e.g., S104–S108) that flag likely hard-coded secrets using heuristic signals, such as credential-shaped strings or suspicious variable names. 
Though limited, these rules expose recurring cues linked to security-sensitive code.
\textbf{Harder best practices}, like those in PEP 506, build on these cues but require additional semantic and contextual reasoning.
Detecting insecure uses of the random module, reliably requires recognizing when these signals co-occur with developer intent, such as credential generation or authentication logic, going beyond what fixed heuristics can capture. 

This defines a difficulty progression in code linting, driven by the increasing contextual and semantic reasoning needed to identify best practice violations. As noted by \citet{chang2025model}, failures to generalize along such progressions arise not from data scarcity, model scale, or inference limits, but from learning paradigms that fix the hypothesis class and inhibit abstraction. Flat supervision maps programs directly to violation labels, forcing models to memorize isolated best practices instead of extracting reusable structure. Although easy violations expose low-level heuristics, current training setups do not elevate these signals into higher-order representations, preventing inductive transfer to harder or novel best practices. In contrast, \textsc{MetaLint} restructures supervision around code idioms, leveraging signals from easy violations to learn semantic abstractions that support detection of harder best-practice violations from high-level specifications.

MetaLint integrates with instruction fine-tuning (IFT) and preference-optimization (PO) methods, leveraging task structure and large-scale synthetic data from existing linters (e.g., Ruff \citep{ruff_linter}, PMD \citep{pmd_analyzer}) to achieve cross-task generalization \citep{Sanh2021MultitaskPT, Wang2022SuperNaturalInstructionsGVA} and improve performance on hard best practices.
Moreover, we construct and publicly release a human-curated benchmark of hard best practices from popular PEPs, in contrast to prior work that builds datasets automatically \citep{holden2024code, zhang2024refactoring, jiang2025coupjava} or does not release them \citep{vijayvergiya2024ai}.
We evaluate state-of-the-art code and reasoning models against \textsc{MetaLint}-trained models to measure their ability to go beyond memorizing easy heuristics.
\textbf{Our key contributions are:}
\begin{enumerate}[itemsep=0pt, leftmargin=*, parsep=0pt, topsep=-5pt, partopsep=0pt]
\item \textsc{MetaLint}, a training framework that bootstraps signals from easy best practices to support inductive transfer to harder or novel practices.
\item Manually curating and releasing a benchmark of hard-to-detect, broadly relevant best practices inspired by PEPs to probe easy-to-hard generalization.
\item \textsc{MetaLint}-trained Qwen3-4B outperforms larger models in detection recall and achieves competitive localization scores to o3-mini without additional test-time compute.
\item Generalization across programming languages (Python, Java), model families (Qwen, Llama), scales (3B–8B), linters (Ruff, PMD, Tree-Sitter) and reasoning settings.
\end{enumerate}
Overall, \textsc{MetaLint} complements rather than replaces linters, showing that organizing supervision around semantic units enables transfer to harder best practices. 
Code linting offers a realistic generalization testbed: correctness is mostly objective, but difficulty ranges from automated verification to context-dependent cases requiring human judgment, making this a first step toward progressively incomplete supervision.

==> sections/001_intro_v2.tex <==
\section{Introduction}
\textit{Code linting}, or static analysis to ensure code complies with best practices, is a fundamental tool for improving software quality and reliability. 
Recent work has explored the use of large language models (LLMs) for best-practice-oriented linting \citep{vijayvergiya2024ai, fang2025lintllmopensourceveriloglinting, holden2024code, khare2023understanding, zhang2024refactoring}, demonstrating improvements over traditional rule-based linters. 
These approaches typically train models to predict violations from a fixed set of best practices.
However, \textbf{best practices are not static: they evolve over time.} \yiqing{use one sentence to describe how it evolves?}\yiqing{I removed "often depend on context" because that's what you talk about in the next paragraph.}
By training the model to map programs directly to violation labels, it only memorizes specific rules seen during training and does not generalize well to rare or unseen best practices \citep{holden2024code}.
Furthermore, the model may over-flag outdated or contextually inappropriate violations, negatively impacting developer experience \citep{vijayvergiya2024ai}. 
% More broadly, the issue stems not only from limited or outdated data, but from the way supervision is structured: mapping programs directly to violation labels encourages rule memorization instead of generalization.

Generalization across best practices becomes especially challenging when considering the varying difficulty of identifying best practices. 
Some violations are relatively \textbf{easy to detect}, relying on surface-level cues. 
For example, linters such as Ruff include rules (e.g., S104--S108) that flag likely hard-coded secrets using heuristic signals like credential-shaped strings or suspicious variable names. 
In contrast, \textbf{harder best practices require contextual and semantic reasoning}. 
For instance, PEP 506 \citep{pep506} recommends using \texttt{secrets.choice} instead of \texttt{random.choice} for security-sensitive applications. 
Detecting such violations requires recognizing both the underlying idiom and the intent of the code, as not every use of \texttt{random.choice} is unsafe. 
This defines a natural difficulty progression in code linting, from heuristic pattern matching to context-dependent reasoning.

\yiqing{Can we somehow merge this paragraph into the previous one? It's still talking about how challenging easy-to-hard generalization is. Also, the "failures to generalize is from the learning paradigm itself" sentence seems to fit better in the first paragraph.}
Failures to generalize across this progression arise not primarily from model scale or data quantity, but from the learning paradigm itself \citep{chang2025model}. 
Current approaches rely on flat supervision over a fixed set of rules, which constrains the hypothesis space and prevents models from forming higher-level abstractions. 
Although easy violations expose useful low-level signals, these signals are not composed into representations that transfer to harder or novel best practices.

To capture the evolving and context-dependent nature of best practices, we \textbf{reframe code linting as meta-learning over \textit{code idioms}}: recurring patterns that capture semantic intent beyond surface syntax. 
In this formulation, best practices correspond to constraints over idioms, and violations arise when problematic idioms appear in contexts where safer alternatives exist. 
For example, recognizing the idiom \texttt{random.choice} is insufficient on its own; models must also infer whether it is used in a security-critical context where \texttt{secrets.choice} is more appropriate. 
By learning to reason over idioms and their contexts, models can move beyond memorizing individual rules and instead generalize to new best practices.

Building on our new problem formulation, we propose \textsc{MetaLint}, a training framework that leverages large-scale synthetic supervision from existing linters to learn idiom-level representations. 
\yiqing{You need to talk about what is the novelty of your MetaLint method. The current narrative sounds like IFT+PO is your novelty (which doesn't sound novel).}
\textsc{MetaLint} integrates with instruction fine-tuning (IFT) and preference optimization (PO), enabling models to detect and localize violations from high-level natural language specifications and examples. 
This structure allows signals from easier, heuristic-based violations to support learning of more complex, context-dependent ones.

To evaluate generalization, we construct and publicly release a human-curated benchmark of hard best practices derived from widely adopted PEPs. 
This contrasts with prior work that either relies on automatically generated datasets \citep{holden2024code, zhang2024refactoring, jiang2025coupjava} or does not release evaluation data \citep{vijayvergiya2024ai}, making it difficult to assess performance on realistic, challenging cases.
Empirically, \textsc{MetaLint}-trained models outperform larger baselines on detecting hard best-practice violations, achieving higher recall while maintaining competitive localization performance to o3-mini even without additional test-time compute. 
These gains hold across programming languages (Python and Java), model families (Qwen and Llama), scales (3B--8B), and underlying linters (Ruff, PMD, and Tree-Sitter), demonstrating strong cross-task and cross-domain generalization.

\yiqing{I'll probably remove this paragraph.}
Overall, \textsc{MetaLint} complements traditional linters by organizing supervision around semantic units rather than fixed rules. 
Code linting thus provides a realistic testbed for studying generalization: while correctness is often objectively verifiable, the difficulty of violations ranges from simple heuristics to complex, context-dependent reasoning, offering a natural setting for investigating learning under progressively incomplete supervision.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{pictures/MetaLint Approach Illustration.png}
\caption{MetaLint frames linting as instruction following, enabling adaptation to novel best practices at test time, whereas prior work maps code to violations within a fixed rule set.}
    \label{fig:meta_lint_approach}
\end{figure*}

==> sections/001_intro_v3.tex <==
\section{Introduction}
\textit{Code linting}, or static analysis to ensure code complies with best practices, is a fundamental tool for improving software quality and reliability. 
Recent work has explored the use of large language models (LLMs) for best-practice-oriented linting \citep{vijayvergiya2024ai, fang2025lintllmopensourceveriloglinting, holden2024code, khare2023understanding, zhang2024refactoring}, demonstrating improvements over traditional rule-based linters by enabling more contextual and semantic reasoning. 

However, existing approaches typically train LLM linters to predict violations from a fixed set of best practices. 
In practice, best practices evolve over time as languages, libraries, and security standards change, leading models trained on static rule sets to over-flag outdated patterns \cite{vijayvergiya2024ai} and underperform on rare or emerging ones \cite{holden2024code}. 
This challenge is compounded by the varying difficulty of identifying violations: some are \textbf{easy to detect}, relying on surface-level cues (e.g., Ruff rules S104--S108 that flag likely hard-coded secrets), while others require \textbf{contextual and semantic reasoning}. 
For example, PEP 506 \citep{pep506} recommends using \texttt{secrets.choice} instead of \texttt{random.choice} for security-sensitive applications, but detecting such violations requires reasoning about code intent, as not every use of \texttt{random.choice} is unsafe.

To address these limitations, we introduce \textsc{MetaLint}, a meta-learning framework that \textbf{formulates code linting as an instruction-following task, instead of static classification}, where each best practice is specified in natural language and treated as a task (Figure~\ref{fig:meta_lint_approach}). 
Unlike fixed-rule classification, this formulation encourages models to move beyond memorizing rule-specific patterns and instead generalize across \textit{code idioms}, or recurring patterns that capture semantic intent beyond surface syntax. 
Inspired by prior work on instruction tuning and cross-task generalization \citep{Sanh2021MultitaskPT, Wang2022SuperNaturalInstructionsGVA}, \textsc{MetaLint} uses a scalable synthetic data pipeline that leverages existing linters (e.g., Ruff \citep{ruff_linter}, PMD \citep{pmd_analyzer}) both as sources of supervision and as reward functions: linters generate labeled data for instruction-following fine-tuning and score candidate outputs to construct preference optimization data via rejection sampling. 
This setup turns abundant, easy-to-obtain heuristic signals into structured supervision that supports transfer to harder and unseen best practices.

To evaluate this generalization, we introduce and publicly release a human-curated benchmark of challenging best practices inspired by widely adopted Python Enhancement Proposals (PEPs). Unlike prior work that relies on automatically generated datasets \citep{holden2024code, zhang2024refactoring, jiang2025coupjava} or does not release evaluation data \citep{vijayvergiya2024ai}, our benchmark targets hard, context-dependent violations and explicitly measures generalization to unseen rules. 
Within this framework, we present the first meta-learning approach to code linting, formulate linting as instruction following rather than fixed-rule classification, and construct synthetic training data that supports both fine-tuning and preference optimization. 

\yiqing{Can we say more about the experiment results? I like the original version where you have numbers. We probably want to emphasize that we observe MetaLint achieves easy-to-hard generalization.}
Empirically, \textsc{MetaLint}-trained models substantially improve performance on hard best practices without explicit fine-tuning, exhibiting strong easy-to-hard generalization. 
These gains hold across programming languages, model families, scales, reasoning settings, and linter sources.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{pictures/MetaLint Approach Illustration.png}
\caption{MetaLint frames linting as instruction following, enabling adaptation to novel best practices at test time, whereas prior work maps code to violations within a fixed rule set.}
\label{fig:meta_lint_approach}
\end{figure*}
